Ordered graphs of bounded twin-width

We consider hereditary classes of graphs equipped with a total order. We provide multiple equivalent characterisations of those classes which have bounded twin-width. In particular, we prove a grid theorem for classes of ordered graphs which have unbounded twin-width. From this we derive that the model-checking problem for first-order logic is fixed-parameter tractable over a hereditary class of ordered graphs if, and -- under common complexity-theoretic assumptions -- only if the class has bounded twin-width. For hereditary classes of ordered graphs, we show that bounded twin-width is equivalent to the NIP property from model theory, as well as the smallness condition from enumerative combinatorics. We prove the existence of a gap in the growth of hereditary classes of ordered graphs. Furthermore, we provide a grid theorem which applies to all monadically NIP classes of structures (ordered or unordered), or equivalently, classes which do not transduce the class of all finite graphs.

==> bound.tex <==
\subsection{Improved lower bound}
We now show that $\CC$ has growth at least 
\begin{align}\sum_{k=0}^{\lceil n/2\rceil}{n \choose 2k}k!=n^{n/2+o(n)}\label{eq:growth}
\end{align}
confirming a conjecture of Balogh, Bollob\'as, and Morris~\cite[Conjecture 2]{BALOGH20061263}.
The proof follows the lines of the proof of Lemma 6 in~\cite{BALOGH20061263},
which states the following.

For a permutation $\pi\from [n]\to[n]$
consider the ordered graph $H(\pi)$ with 
vertex set $[2n]$, ordered naturally, where vertex $i$ is adjacent with vertex $\pi(i)+n$,
for each $i\in[n]$. 

\begin{lemma}[\cite{BALOGH20061263}]\label{lem:balogh}
    Let $\CC$ be a hereditary class of ordered which contains all ordered graphs of the form $H(\pi)$, for all $n\in\N$ and permutations $\pi$ of $[n]$.
    Then $\CC$ has growth at least~\eqref{eq:growth}.
\end{lemma}

Suppose $\CC$ is a hereditary class of graphs which contains $\regsigma$, for some $\sigma\in\schemes$.
Then $\sigma$ specifies one of four types in $\set{\le,\ge,=,\neq}$.
We only need to consider two cases, say of $\le$ and $=$, as the others follow by symmetry or edge complementation.

The case of $=$ follows from
Lemma~\ref{lem:balogh}.
Indeed, we show that $\CC$ contains every ordered graph of the form $H(\pi)$.

Pick a permutation $\pi$ of $[n]$,
and consider the $(n-1)\times (n-1)$ regular semigrid in $G\in \regsigma$ (recall that $\sigma$ imposes the type $=$)
with intervals $I_0,I_1,\ldots,I_{n}$ of size $n+1$ each.
Assume that $\sigma$ specifies $I_0<I_1<\ldots<I_{n}$, otherwise reverse the order, and arrange the intervals into the $[n+1]\times [n+1]$ matrix as done in the definition of regular semigrids.
Let $G_\pi$ be the substructure of $G$ induced by $\set{0}\times [n-1]\cup \setof{(\pi(i),i)}{i\in[n]}$.

For each $i\in[n]$, the vertex $(0,i)$ is adjacent only to $(\pi(i)+1,i)$ in $G_\pi$,
and $(\pi(i)+!,i)$ is the $n+\pi(i)$-th smallest vertex in $G_\pi$ (recall that the order $\le $ on $[n+1]\times [n+1]$ is lexicographic).
Hence, $G_\pi$ is isomorphic to $H(\pi)$.\todo{pic}

By Lemma~\ref{lem:balogh}, $\CC$ has growth at least as in~\eqref{eq:growth}, in case when $\CC$ contains arbitrarily large regular semigrids of  type $=$.









==> junk.tex <==

	A similar characterization to~\eqref{it:grid-or}  appears in~\cite{bonnet2020twinwidth}. There it is shown that for a class of \emph{unordered} graphs $\CC$, the following are equivalent:
    \begin{enumerate}
        \item[1'.] $\CC$ has bounded twin-width,
        \item[2'.] there is $t\in \N$ such that 
        for every $G\in\CC$ there is an ordering $\le$ such that for every two convex partitions $\cal L,\cal R$ of $V(G)$ into $t$ parts each, there are $L\in\cal L$ and $R\in\cal R$ such that $L$ is $1$-simple over $R$ or $R$ is $1$-simple over $L$.
    \end{enumerate}
    This equivalence also holds for classes of ordered graphs, but the order obtained in (2') is not necessarily the same order as the order in the graph, and changing the order cannot be avoided in some cases. For example, 
    consider the class $\CC$ of complete bipartite graphs $K_{n,n}$ ordered so that the successor of a vertex in one part is in the other part.
    Then $\CC$ is a class of ordered graphs of bounded twin-width, but for every $t\in\N$ the graph $K_{t,t}$ 
    partitioned into $t$ intervals of size $2$ is such that no part is $1$-simple over another. 
    

\begin{comment}


    \section{Order-invariant transductions}\todo{do something}
    Fix a signature $\Sigma$ and a class $\CC$ of $\Sigma$-structures.
    A sentence $\phi$ over the signature $\Sigma\cup\set\le$
    is called \emph{order-invariant} on $\CC$ if for all $\str A\in\CC$,
    the truth value of $\phi$ in $\str A$ expanded by an order $\le$ does not depend on the choice of the order $\le$. We now extend this notion to transductions.
    
    Let $\Sigma$ and $\Gamma$ be relational signatures.
    A \emph{interpretation} $I\from\Sigma\to\Gamma$ consists of a $\Sigma$-formula $\delta(x)$ and for each symbol $R\in \Gamma$ of arity $k$, a $\Sigma$-formula $\phi_R(x_1,\ldots,x_k)$.	
    Given a $\Sigma$-structure $\str A$, define $I(\str A)$ as the $\Gamma$-structure with domain $D=\delta(\str A)$ equipped with the relations $\phi_R(\str A)$ restricted to $D$, for each $R\in\Gamma$.
    
    % A  \emph{transduction} $T\from\Sigma\to\Gamma$ 
    % is a $\widehat\Sigma$-interpretation for some $\widehat\Sigma$ extending $\Sigma$ by unary predicates.
    % Given a $\Sigma$-structure $\str A$, define $I(\str A)$ as the set of $\Gamma$-structures $I(\widehat{{\str A}})$, where $\widehat{\str A}$ ranges over all $\widehat\Sigma$-structures expanding $\str A$.
    
    A class of $\Gamma$-structures $\DD$ is a \emph{transduction} of a class of $\Sigma$-structures $\CC$ if there is a transduction $T\from\Sigma\to\Gamma$ 
    such that for every structure $\str D\in\DD$ there is some $\str C\in\CC$ with $\str D\in T(\str C)$.
    A class of $\Gamma$-structures $\DD$ is an \emph{order-invariant} transduction of a class of $\Sigma$-structures $\CC$ if there is a transduction 
    $T\from \Sigma\cup\set{\le}\to \Gamma$ such that for every structure $\str D\in\DD$ there is some $\str C\in\CC$ such that 
    $\str D\in T(\str C_\le)$
    for every expansion $\str C_\le$ of $\str C$ by an order $\le$.
    
    Above, all formulas (in the definition of an interpretation) are assumed to be first-order formulas. 
    If in the above definitions we allow MSO formulas rather than first-order formulas, then we may speak of MSO transductions etc. 
    
    \begin{theorem}For every class of finite, binary structures $\CC$, exactly one of the following conditions holds:
        \begin{itemize}
            \item $\CC$ has bounded twin-width, or
            \item the class of all finite graphs is an  order-invariant transduction of $\CC$.
        \end{itemize}
    \end{theorem}
    
    
    As order-invariant MSO transductions extend CMSO transductions, we have an analogous result for cliquewidth and MSO.
    \begin{theorem}For every class of finite, binary structures $\CC$, exactly one of the following conditions holds:
        \begin{itemize}
            \item $\CC$ has bounded cliquewidth, or
            \item the class of all finite graphs is an order-invariant MSO transduction of $\CC$.
        \end{itemize}
    \end{theorem}
    
    \end{comment}
